On barren plateaus and cost function locality in variational quantum algorithms

Variational quantum algorithms rely on gradient based optimization to iteratively minimize a cost function evaluated by measuring output(s) of a quantum processor. A barren plateau is the phenomenon of exponentially vanishing gradients in sufficiently expressive parametrized quantum circuits. It has been established that the onset of a barren plateau regime depends on the cost function, although the particular behavior has been demonstrated only for certain classes of cost functions. Here we derive a lower bound on the variance of the gradient, which depends mainly on the width of the circuit causal cone of each term in the Pauli decomposition of the cost function. Our result further clarifies the conditions under which barren plateaus can occur.

==> on_designs.tex <==
\section{An informal introduction to measures and $t$-designs}

Let us first discuss probability theory on the unitary group $U(d)$. Probability theory uses the following construction. Let $\Omega$ be the sample space, $\mc{F}$ be a $\sigma$-algebra of subsets of $\Omega$ (meaning that $\mc{F}$ is closed under complement and countable unions). Then $P$ is a \textit{probability measure}, i.e. a function $\mc{F} \rightarrow [0, 1]$ with the properties that you might expect: $P(\Omega) = 1$, countable additivity, and $P(\varnothing) = 0$. This elaborate construction is needed to unify the discrete and continuous probability theory, and to avoid dealing with tricky questions like sets with undefined Lebesgue measure.

In our case, $\Omega = U(d)$, $\mc{F}$ is the system of so-called Borel sets (the set of all open spheres, which are then subject to countable unions and intersections). Now we can introduce the \textit{Haar measure} $\mu: \mc{F} \rightarrow [0, 1]$. The defining property of that measure is that for any Borel set $\mc{A}$, its measure is conserved under translation with any unitary $U$: $\mu(U\mc{A}) = \mu(\mc{A}) = \mu(\mc{A}U)$. The existence and uniqueness of this measure is a nontrivial fact (see \cite{watrous_theory_2018} for more details). This measure can be thought of as ``the most uniform'' probability distribution on $U(d)$.

It is known that sampling from the Haar measure using quantum circuits is exponentially hard [Knill 1995]. Thankfully, for some applications, we can be satisfied with less. Given a random unitary $U$, we can construct other random variables out of its individual entries $u_{ij}$. We will call a polynomial a $(t, t)$-polynomial if its monomials are comprised of no more than $t$ entries of $U$ and no more than $t$ entries of $U^*$ (complex conjugate, not Hermitian conjugate). For example, given a matrix $A$, the expression $\Tr U^\dagger A U$ = $\sum_{i, j, k} u^*_{ji} a_{jk} u_{ki} $ is a $(1, 1)$-polynomial.

If we only care about the expected values of such polynomials, we can safely replace the Haar measure by some other random distribution which is easier to sample. A measure $\nu$ is an exact $t$\textit{-design} if for any $(t, t)$-polynomial $f(U)$, the expected value $\mathbb{E}_\nu f$ with respect to $\nu$ is the same as the expected value $\mathbb{E}_\mu f$ with respect to the Haar measure.

For example, the Clifford group forms an exact $3$-design, and sampling from this group requires a polynomially-deep quantum circuit.

Finally, we can go even further and approximate these designs too. To discuss the notion of an approximate $t$-design, we introduce the following quantum channel:

$$
\Delta_{\mu,t} [X] = \int d\mu(U) (U^\dagger)^{\otimes t} X (U^\dagger)^{\otimes t}, \ X \in \mathrm{Herm}(d^t).
$$
 
A similar channel can be introduced for any measure. For these channels we can introduce the superoperator norm (analogous to the operator norm for regular operators). This yields the definition of an $\epsilon$-approximate \textit{t-copy tensor product expander}, which is a measure $\nu$ such that $|| \Delta_{Haar,t} - \Delta_{\nu,t}|| < \epsilon$.

Another way of comparing the channels is based on complete positivity. Write $\mc{N}_1 \preceq \mc{N}_2$ if $\mc{N}_2 - \mc{N}_1$ is a completely positive operator. Then $\nu$ is an $\epsilon$-approximate $t$-design if

$$
(1- \epsilon) \Delta_{Haar,t} \preceq \Delta_{\nu,t} \preceq (1 + \epsilon) \Delta_{Haar,t}.
$$

These definitions are used by Refs. \cite{brandao_local_2016,harrow_approximate_2018} to prove that approximate $t$-designs can be created by a circuit of depth $\mc{O}(t^{10} n)$.

There are other definitions of an approximate $t$-design. For example, one can define the proximity to an exact $t$-design simply as a superoperator norm \cite{Low_2010}: $||\Delta_{\nu, t} - \Delta_{Haar, t}||_\diamond < \epsilon$.

==> outtakes.tex <==
\newpage

\section*{OUTTAKES}

\textbf{Below are bits that can be possibly included in the main text but are currently out of place. Also includes lemmas that ended up not being necessary for the final text.}

For a while, let us remember that $[iF, H]$ is a Hermitian operator for Hermitian $F, H$ and omit the commutator that appears in (\ref{eq:partial_E}). If we also suspend the randomness of $U_A$ for a while, this means that we are effectively interested in evaluating the following expression:

\begin{multline}
\label{eq:problem_simplified}
    \mathrm{V} = \int d\nu (U) \bra{\mathbf{0}}U^\dagger H U \ket{\mathbf{0}}^2 = \\
    = \int d\nu (U) (\bra{\boldsymbol{0}} \otimes \bra{\boldsymbol{0}})
    (U^\dagger \otimes U^\dagger)
    (H \otimes H)
    (U \otimes U)
    (\ket{\boldsymbol{0}} \otimes \ket{\boldsymbol{0}})
\end{multline}

for some Hermitian $H$ acting on $\mathcal{H}$. The reason to write this as a long tensor product expression is the following. Suppose $U$ is distributed as a local 2-design acting on some subsystem $\mathcal{Y}$. Then, by substituting the variables into (\ref{eq:int_haar_swap}), we obtain:

\begin{multline}
    \label{eq:local_2_design}
    \int d\nu (U)
    (U^\dagger \otimes U^\dagger)
    (H \otimes H)
    (U \otimes U)
    = \frac{1}{\mathrm{dim} \mc{Y}^2 - 1} \cdot \\
    \cdot \left[ \left(\Tr_\mc{Y, Y'} (H \otimes H) - \frac{1}{\mathrm{dim} \mc{Y}}\Tr_\mc{Y, Y'} \mc{S_\mc{Y, Y'}} (H \otimes H)  \right) \otimes \mathbbm{1}_{\mc{Y, Y'}} + \right. \\
    \left.  +  \left(\Tr_\mc{Y, Y'} \mc{S_\mc{Y, Y'}} (H \otimes H) - \frac{1}{\mathrm{dim} \mc{Y}}\Tr_\mc{Y, Y'}  (H \otimes H)  \right) \otimes \mc{S}_{\mc{Y, Y'}}\right].
\end{multline}{}

Here $\mc{S}_{\mc{Y, Y'}}$ means a swap operator that switches the two copies of the subsystem $\mc{Y}$. 

As a result, the output of the formula is an operator acting on $(\mc{H}\otimes \mc{H})$, which also intertwines the copies. That is why we choose to always work with pairs of operators\footnote{Perhaps we might want to call this ``double operators'' or something.}. 

We can now introduce a superoperator acting on $\mc{L} (\mc{H}\otimes \mc{H})$:

 The precise action of this superoperator is shown in (\ref{eq:local_2_design}).


Now, if we want to compute the second moment of $\langle h \rangle$ over some ansatz consisting of $N$ building blocks with domains $\mc{Y}_1, ..., \mc{Y}_N$, we simply compute 
\begin{equation}
    \hat{O} = M_{ \mc{Y}_N} \circ \dots \circ  M_{ \mc{Y}_1} (h \otimes h),
\end{equation}
provided that each block is a local 2-design.
Then we ``hug'' the result with zero vectors: $(\bra{\boldsymbol{0}} \otimes \bra{\boldsymbol{0}}) \hat{O} (\ket{\boldsymbol{0}} \otimes \ket{\boldsymbol{0}})$.


\section{Probabilistic point of view}

In this section, we take advantage of the fact that 

$$
s = \frac{1}{2}(X \otimes X + Y \otimes Y + Z \otimes Z + 1 \otimes 1) 
\equiv \frac{1}{2}(x + y + z + 1).
$$

One can notice that for $d=2$, it is true that 
$$
\frac{1}{d^2 - 1}(ds -1) = \frac13(x + y + z).
$$
A similar fact can be shown for 2-local channels:
\begin{equation}
    \frac{1}{d^4 - 1}(d^2 ss - 11) = \frac{1}{15}((x + y + z + 1)(x+y+z+1) - 11).
\end{equation}
In other words, one can formulate the problem in the following equivalent way:
each local 2-design corresponds to a probabilistic channel $\Phi$ that replaces any nontrivial paired Pauli string with a random nontrivial Pauli string. After applying them all in the order dictated by the ansatz, what is the probability that the output consists entriely of 1's and $z$'s? We claim that the following is true:

\begin{equation}
\label{eq:future_cone}
    \mathrm{V} \geq \left( \frac{1}{5} \right)^{\#blocksFC},
\end{equation}
where $\#blocksFC$ is the number of blocks in the first layer of the ansatz, such that the domain of $U^\dagger H U$ can intersect their domain for some realization of the ansatz $U$. For a checkerboard ansatz with $L$ layers and initial locality $l$, we can estimate $\#blocksFC \leq l\cdot L$.

The proof is easy: in the worst case, the Pauli matrices ``contaminate'' all qubits in the future cone. Then for each two-qubit block, only 3 of 15 possibilities yield nonzero result, these are $z1, zz, 1z$. However, if some block in the past yields, for example, $1x$, then the next block that shares the left qubit with that guy would receive $11$ as input and leave in untouched. Hence Eq. \ref{eq:future_cone} is a lower bound.


Finally, we make a very important observation:

\begin{proposition}


\label{thm:all_are_ids_and_swaps}
Let $\mc{Y}_1, ..., \mc{Y}_N$ be a set of subsystems that can cover $\mc{H}$ (overlaps are allowed). Then, for any $H \in \mathrm{Herm}(\mc{H})$, the combined action of 
$ M_{ \mc{Y}_1}, ..., M_{ \mc{Y}_N}$ on $H$ returns a sum of terms consisting exclusively of local identity operators and swap operators permuting the copies of some subsystem:
\begin{equation}
    \label{eq:ids_and_swaps}
     M_{ \mc{Y}_N} \circ \dots \circ  M_{ \mc{Y}_1} (H \otimes H) 
     = \sum_{\mc{A} \cup \mc{B} = \mc{H}} C_{\mc{A}, \mc{B}} 
     \mathbbm{1}_{\mc{A},\mc{A'}} \mc{S}_{\mc{B}, \mc{B'}}, 
     \quad C_{\mc{A}, \mc{B}} \in \mathbb{R}.
\end{equation}{}
In this sum, $\mc{A}$ and $\mc{B}$ are only allowed to span some qudit subsets.
\end{proposition}
Note that for evaluating $\mathrm{V}$, we only care about the sum of the coefficients $C_{\mc{A}, \mc{B}}$ themselves.
\begin{proof}
Let us begin by decomposing $H$ into a sum of Pauli strings:
$$
H = \sum_{\gamma \in \{0, 1, 2, 3\}^{\times n}} c_\gamma \sigma_{\gamma_1} \otimes ... \otimes \sigma_{\gamma_n}, c_\gamma \in \mathbb{R}.
$$
Here $\gamma$ is a multiindex enumerating the possible Pauli strings. For qudits with $d>2$, one should use Hell-mann matrices instead of Pauli matrices, but all other reasoning is exactly the same, so we will focus on $d = 2$.

$H \otimes H$ now consists of $(\mathrm{Card} (H))^2$ Pauli strings. All $M_{\mc{Y}_i}$ operators are linear, hence we can keep track of each of the strings separately. If the domains $\mc{Y}_1, ..., \mc{Y}_N$ do not overlap, then in each subsystem $M_{\mc{Y}_i}$ transforms the Pauli operators into a linear combination of identity and swap operators in $\mc{Y}_i, \mc{Y'}_i$, and the theorem is proven. If the domains do overlap, then some $M_{\mc{Y}_j}$ receives a combination of identities, swap gates and Pauli operators. This complicated input can still be traced out over $\mc{Y}_j, \mc{Y'}_j$, so by (\ref{eq:local_2_design}) any term in the output only has identities and swaps in this subspace. As long as the domains cover the entire Hilbert space $\mc{H}$, no subspace will be left unaffected.
\end{proof}{}


\begin{lemma}
\label{lemma:1-designs_stack}
If $W$ and $V$ are unitary 1-designs with probability measures $\omega$ and $\nu$, then $W \otimes V$ is also a unitary 1-design. An equivalent statement for 2-designs is \emph{not} true.
\end{lemma}

\begin{proof}
% Let $U$ and $V$ be independent 1-designs. This means that integrating an expression like $\int U A U^\dagger d\omega(U)$ is the same as integrating over the Haar measure, that is:
Use Lemma \ref{lemma:int_haar} to verify the statements explicitly:

\begin{multline}
    \int (W \otimes V) (A \otimes B) (W^\dagger \otimes V^\dagger) d\omega(W) d \nu (V) = \\
    = \frac{\Tr A \Tr B}{\dim W \dim V} \mathbbm{1} \equiv \int U (A \otimes B) U^\dagger d\mu(U).
\end{multline}{}

% Consider the expression $\int (U A U^\dagger) \otimes (V B V^\dagger) d\omega(U) d\nu(V)$. This is equal to $1/(d_A d_B) \Tr A \Tr B$, which is exactly the same as if $\int W (A \otimes B) W^\dagger d\mu_{Haar} (W)$ for $W \in U(d_A d_B)$. To make sure that the same logic does not apply to 2-designs, one instead should compare expressions of the type $\int U^{\otimes 2} C (U^\dagger)^{\otimes 2} d\omega(U)$.

For 2-designs, the reader can check that the expression 
$ \int (W \otimes V)^{\otimes 2} (A \otimes B)^{\otimes 2} (W^\dagger \otimes V^\dagger)^{\otimes 2} d\omega(W) d \nu (V)$ does not decouple in the same easy fashion.

\end{proof}{}



Another interesting fact:
\begin{proposition}
\label{prop:m2_is_proj}
$M_{\mc{Y}}$ is a projector. The $+1$ eigenspace of that projector, narrowed down to $\mathcal{L}(\mc{Y} \otimes \mc{Y'})$, is spanned by $\mc{S}_{\mc{Y, Y'}}$ and $\mathbbm{1}_{\mc{Y, Y'}}$.
\end{proposition}{}
\begin{proof}
Check that $M_{\mc{Y}} \circ M_{\mc{Y}} = M_{\mc{Y}}$. Then see by inspection that $\mc{S}_{\mc{Y, Y'}}$ and $\mathbbm{1}_{\mc{Y, Y'}}$ are $+1$ eigenfunctions of $M_{\mc{Y}}$. To see that there are no other linearly independent eigenfunctions, consider $u = \alpha sss + \beta 111 + \gamma v$, where $v$ is orthogonal to both of these in terms of the Hilbert-Schmidt inner product. Apply $M$ to this and see that $\gamma$ is necessarily zero.
\end{proof}{}


\begin{proposition}
$M_\mc{Y}$ is trace-preserving.
\end{proposition}{}
\begin{proof}
Observe that taking a trace commutes with integration over the unitaries. In the tracing, $U$ and $U^\dagger$ will eliminate each other, leaving use with a trace of the original operator. By normalization condition, $\int dU = 1$.
\end{proof}{}


Denote a paired Pauli string as $\left\{\begin{array}{c}
     X Y Z Y Z Y\\
     X Y Z Y Z Y
\end{array}{}\right\}
$.

\section{Everything I know for sure about the mixing operator}

Denote $M^m$ the mixer on $m = i + j + k + l$ pairs of qubits.

\begin{multline}
M^{i + j + k + l} (1...1\sigma ... \sigma s...s \varphi ... \varphi) = \\
= ?
% = \frac{1}{4^{i + j + k + l} - 1} 
% \left( (\Tr 1)^i \right)
\end{multline}{}

Consider the following:

\begin{multline}
    C_1 = \Tr (1...1\sigma ... \sigma s...s \varphi ... \varphi) = 4^i 0^j 2^k 0^l; \\ 
    C_2 = \Tr s...s (1...1\sigma ... \sigma s...s \varphi ... \varphi) = 2^i 2^j 4^k 2^l; \\
    M^{m} (1...1\sigma ... \sigma s...s \varphi ... \varphi) = \\
    = \frac{1}{4^m - 1} 
    \left( (C_1 - \frac{1}{2^m} C_2)1...1 
    + (C_2 - \frac{1}{2^m} C_1)s...s\right).
\end{multline}{}

In particular:

\begin{tabular}{|c||c|c|c|c|c||c|c||c|}
    \hline
     input of $M$ & $m$ & $i$ & $j$ & $k$ & $l$ & $C_1$ & $C_2$ & result \\
    \hline
     1 & 1 & 1 & 0 & 0 & 0 & $4$ & $2$ & 1 \\
     $\sigma$ & 1 & 0 & 1 & 0 & 0 & $0$ & $2$ & $\varphi$ \\
     $s$ & 1 & 0 & 0 & 1 & 0 & $2$ & $4$ & $s$ \\
     $\varphi$ & 1 & 0 & 0 & 0 & 1 & $0$ & $2$ & $\varphi$ \\
     \hline
     $11$ & 2 & i & j & k & l & $C_1$ & $C_2$ & 11 \\
     $1 \sigma$ & 2 & i & j & k & l & $C_1$ & $C_2$ & result \\
     $1s$ & m & i & j & k & l & $C_1$ & $C_2$ & result \\
     $1 \varphi$ & m & i & j & k & l & $C_1$ & $C_2$ & result \\
     $\sigma \sigma$ & m & i & j & k & l & $C_1$ & $C_2$ & result \\
     $\sigma s$ & m & i & j & k & l & $C_1$ & $C_2$ & result \\
     $\sigma \varphi$ & m & i & j & k & l & $C_1$ & $C_2$ & result \\
     $ss$ & m & i & j & k & l & $C_1$ & $C_2$ & $ss$ \\
     $s \varphi$ & m & i & j & k & l & $C_1$ & $C_2$ & result \\
     $\varphi \varphi$ & m & i & j & k & l & $C_1$ & $C_2$ & result \\
     
     \hline
     $1...1\sigma...\sigma$ & $i + j$ & $i$ & $j \neq 0$ & 0 & 0 & $0$ & $2^{i + j}$ & $\frac{1}{4^{m}-1} (2^{m}s...s - 1...1)$ \\

     expression & m & i & j & k & l & $C_1$ & $C_2$ & result \\
    \hline
\end{tabular}{}


\section{One layer of the ansatz}

We will start by simplifying the problem as much as possible: let us assume that the ansatz consists of one layer of blocks acting on qudits $\{1, 2\}, \{3, 4\}, \dots, \{2\xi-1, 2\xi\}$ (one layer of the checkerboard ansatz aka alternating layer ansatz aka parallel local circuit). For now, set $n$ to be even. We will also assume that each of these blocks forms a 2-design and that the derivative $\partial_a$ is taken with respect to a parameter in a gate that has no gates after it. The latter allows us to set $U_A = \mathbbm{1}$:


\begin{equation}
    \label{eq:partial_no_u_after}
    \partial_a E = \bra{\mathbf{0}}U^\dagger_B [iF_a, H_0] U_B \ket{\mathbf{0}}.
\end{equation}

Now, $H = [iF_a, H_0]$ is a Hermitian operator, and Eq. \ref{eq:partial_no_u_after} simplifies even further. Decompose $H$ into a weighted sum of Pauli strings: $H = \sum_i c_i h_i, c_i \in \mathbb{R}$\footnote{W.l.o.g. assume that $H$ is traceless.}. Then, we arrive at the following:

\begin{equation}
    \label{eq:variance}
    \Var \partial_a E = \int d\nu (U_B) \sum_{i, j} c_i, c_j \bra{\mathbf{0}}U^\dagger_B h_i U_B \ket{\mathbf{0}} \bra{\mathbf{0}}U^\dagger_B h_j U_B \ket{\mathbf{0}}.
\end{equation}{}



\begin{lemma}
\label{lemma:single_layer_e_2}
Let $H = \sum c_i h_i$ be a traceless Hermitian operator on $\mc{H}$, and $h_i$ be different Pauli strings. Let $U_B$ have the structure of one layer of the checkerboard ansatz, and each block be an independent 2-design. Then,

\begin{equation}
    E_2  \equiv \langle (\bra{\boldsymbol{0}} U_B^\dagger H U_B \ket{\boldsymbol{0}})^2 \rangle_{\nu(U)}
    = \sum_i c_i^2 (d^2 + 1)^{-k(i)},
\end{equation}{}
where $k(i)$ is the number of blocks in $U_B$ whose support overlaps $\operatorname{supp}(h_i)$.

\end{lemma}{}

\begin{proof}


Since we assumed that each block in the ansatz is a 2-design, all we need is apply Eq. \ref{eq:int_haar} to Eq. \ref{eq:variance}. Here we essentially integrate the Pauli matrices in each pair of qubits simultaneously: there are two copies of each qudit, and the traces in Eq \ref{eq:int_haar} can only connect the two copies between each other, not distinct qudits. Let us consider, for example, the pair of qudits $\{ 1, 2 \}$. Keep in mind that the unitaries act on two qudits, hence $\dim U = d^2$. There are several possibilities:

\begin{enumerate}
    \item In both Pauli strings $h_i$ and $h_j$, there are identity matrices in the slots 1 and 2. In this case, $A=B=\mathbbm{1}_{d^2}$, therefore $\Tr A = \Tr B = \Tr AB = d^2$, and the integration yields $\frac{1}{d^4 - 1}((d^4 - 1) \mathbbm{1} \otimes  \mathbbm{1}) = \mathbbm{1}_{d^2}$.
    \item One Pauli string has identity matrices in slots 1 and 2, another one has some Pauli matrix in either slot. In this case $\Tr B = 0$, and the \textit{entire term} for $h_i$ and $h_j$ vanishes.
    \item Both Pauli strings have some Pauli matrices in these slots. Again, unless the Pauli matrices in $h_i$ and $h_j$ match, there will be a trace of some traceless operator in each summand, eliminating the expression. When they do match, $A = B = \sigma_\alpha \otimes \sigma_\beta$. Traces of $A$ and $B$ still vanish, but $\Tr AB = d^2$, hence we obtain 
    $\frac{1}{d^4 - 1}(-\mathbbm{1}_{d^2} + d^2 \mc{S})$.
    \item For both strings, these slots are of the form $\mathbbm{1} \otimes \sigma_\alpha$. Just like in the previous case, $\Tr AB = d^2, \Tr A = \Tr B = 0$, and the result is the same.
\end{enumerate}{}

Same applies to all qubit pairs. Points 2 and 3 imply that the sum in Eq. \ref{eq:variance} only has nonvanishing terms when $i=j$. Finally, note that 

\begin{equation}
\label{eq:hug_with_zeros}
   (\bra{0} \otimes \bra{0}) \mathbbm{1}_{d^2} (\ket{0} \otimes \ket{0}) = (\bra{0} \otimes \bra{0}) \mc{S} (\ket{0} \otimes \ket{0}) = 1. 
\end{equation}{}

Let $k(i)$ denote the number of qudit pairs in which cases 3 or 4 occur for the Pauli string $h_i$. Then, combining all the evidence together, we obtain

\begin{equation}
    \label{eq:simple_variance}
    E_2 = \sum_i c_i^2 \left(\frac{d^2 - 1}{d^4 - 1} \right)^{k(i)} 
    = \sum_i c_i^2 (d^2 + 1)^{-k(i)}.
\end{equation}{}

\end{proof}{}


I think we can safely generalize this a little bit more. Suppose that we had not the checkerboard ansatz, but instead the unitary gates covered all qubit register in arbitrary non-overlapping patches with area $A(p)$. Then the summand for $h_i$ would obtain a multiple $(d^{A(p)} + 1)^{-1}$ for each patch $p$ that overlaps with the support of $h_i$.

\subsection{Case study: a very nonlocal Hamiltonian}

Consider $H_0 = Z \otimes ... \otimes Z$. Unlike the $n$-local projector studied in (Cerezo et al 2020), this Hamiltonian consists of a single Pauli string. Nonetheless, we argue that this Hamiltonian is also susceptible to the barren plateau issue. If we only care about the last-operator derivatives, like above, then the onset of the plateau is easy to show. However, let's look at a slightly more complicated case when $U_A \neq \mathbbm{1}$.

\begin{proposition}
Let $H_0 = Z \otimes ... \otimes Z$ be a Hamiltonian acting on $n$ qubits. Let the ansatz be one layer of parallel 2-local gates acting on consequent pairs of qubits. Let the gate in pair $p = (2l-1, 2l)$ be of the form $U_A^{p} e^{-iF \theta} U_B^(p)$, where $F^2 = 1$ is some Hermitian operator and $U_A^{p}$ and $U_B^{p}$ form independent 2-designs. Then

\begin{equation}
    \langle (\bra{\boldsymbol{0}} U_B^\dagger [iF, U_A^\dagger H_0 U_A] U_B \ket{\boldsymbol{0}})^2 \rangle_{\nu(U)} \in O(\frac{1}{2^n}).
\end{equation}{}
\end{proposition}{}

Demanding that $U_A$ is also a local 2-design is a serious constraint, meaning that $e^{iF}$ is sandwiched somewhere in the middle of the block. Alternatively, we can let it be arbitrary and then upper bound it, so that the average over any distribution of $SU(4)$ is safe.

\begin{proof}
\textbf{This is actually a rough sketch, not proof, but I'm fairly confident that this works.}
To do this, we need to consider the action of $\int U_A^{\otimes 2} \otimes (U_A^{\dagger})^{\otimes 2} d\mu_{Haar} (U)$ as a quantum channel. This will replace Paulis with SWAP operations on the affected qubits. Then we can either decompose SWAPs into Pauli strings or use something else about the commutators.

Then $[iF, \cdot]$ is also kind of a quantum channel (we will need to apply it twice as the value of interest is squared). The commutator will introduce some factor, but it does so just once\footnote{Perhaps the locality of $F$ is relevant, but we'll stick with 2 for now.}. After all these fancy operations, we should end up with no more that three Pauli strings, each exhibiting a barren plateau.
\end{proof}{}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth,angle=90]{ZZZZ_d.jpg}
    \caption{Value to be averaged over random blocks, expressed as a tensor network. In this figure, the wires actually mean two-qubit subspaces, and the derivative is in the first block. In the center, there is the Pauli string $H_0$, which is then conjugated by $U_A$, then commuted with $iF$ (here commutation is expressed as an operator $[iF, \cdot]$, drawn as a $\Pi$-shaped clip). After these two operations, we have a collection of Pauli strings subject to the treatment of Section 4.
    }
    \label{fig:ZZZZZZZ}
\end{figure}{}

We can now instantly show another Hamiltonian which has essentially the same plateau properties despite being only algebraically $n/2$-local.

\begin{corollary}
$H = Z \otimes \mathbbm{1} \otimes Z \otimes \mathbbm{1} \otimes \dots \otimes Z \otimes \mathbbm{1}$ demonstrates the same scaling of the gradient variance as $H_0 = Z \otimes \dots \otimes Z$, up to a constant factor.
\end{corollary}{}

***



% \begin{equation}
% \begin{aligned}
%     \label{eq:m2}
%     & M_{ \mc{Y}} (h_1 \otimes h_2) = \frac{1}{d^{2 |\mc{Y}|} - 1} \cdot
%      \\
%     & \cdot \left[ \left(\Tr_\mc{Y, Y'} (h_1 \otimes h_2) - \frac{1}{d^{|\mc{Y}|}}\Tr_\mc{Y, Y'} \mc{S_\mc{Y, Y'}} (h_1 \otimes h_2)  \right) \mathbbm{1}_{\mc{Y, Y'}} \right. \\
%     & \left.  +  \left(\Tr_\mc{Y, Y'} (h_1 \otimes h_2) - \frac{1}{d^{|\mc{Y}|}}\Tr_\mc{Y, Y'} \mc{S_\mc{Y, Y'}} (h_1 \otimes h_2)  \right) \mc{S}_{\mc{Y, Y'}}\right].
% \end{aligned}{}
% \end{equation}{}

Here $\mc{S}_{\mc{Y, Y'}}$ is the swap operator permuting the subsystems $\mc{Y, Y'}$, which are two copies of the same subsystem. This operator outputs the operator that we obtain by averaging $(U^\dagger h_1 U) \otimes (U^\dagger h_2 U)$ over a Haar-random unitary $U$ acting on $\mc{Y}$. This operator is convenient for the following reason. Suppose we consider an ansatz consisting of $N$ Haar-random gates with supports $\mc{Y}_1, \dots \mc{Y}_N$. 

***

We can also check how this operator acts on all interesting inputs. Especially we want to also look at 
$M_{\mc{Y}}(\mathbbm{1}_\mc{V, V'} \otimes \mc{S}_{\mc{W, W'}})$ for $\mc{Y}= \mc{V} \otimes \mc{W}$. For example, this situation happens if the unitary acts on qubits 2, 3, and we prevoiusly obtained an identity on qubits $2, 2'$ and a swap on qubits $3, 3'$. Direct inspection shows that any other relevant input yields a prefactor smaller that one. Specifically,

\begin{equation}
    \label{eq:m2_id_swap}
    M_{\mc{Y}}(\mathbbm{1}_\mc{V, V'} \otimes \mc{S}_{\mc{W, W'}}) = 
    \frac{d}{d^2+1} (\mathbbm{1}_\mc{Y, Y'} + \mc{S}_\mc{Y, Y'}).
\end{equation}{}

Now, after the first layer of the checkerboard ansatz, any Pauli string $h_i \otimes h_i$ turns into a sum of terms which only consist of identities and swaps. As seen from Eq. \ref{eq:hug_with_zeros}, all such terms yield a $1$ when hugged with $\ket{0}$ vectors. Thus the problem reduces to accounting for the sum of the prefactors.

Deinfe $\alpha = \frac{1}{d^4 - 1}, \ \beta=\frac{d}{d^2+1}$. Now, suppose we've attacked the desired Pauli string with one layer of the ansatz. From Eq. \ref{eq:simple_variance} we see that the result is a sum of operators consisting of identities and swaps, with the sum of coefficients equal to $\alpha^k (d^2 - 1)^k$. What happens if we apply more blocks of the ansatz? If $M_2$ hits a pair of qubits with identity or swap on both of them, nothing changes, as follows from Proposition \ref{prop:m2_is_proj}. The only other possible situation is that shown in Eq. \ref{eq:m2_id_swap}. In which case, the overall sum gets a prefactor of at least $2 \beta$. Overall, this lets us impose a loose lower bound on the total value of $S = (\bra{\boldsymbol{0}} \otimes \bra{\boldsymbol{0}}) \hat{O} (\ket{\boldsymbol{0}} \otimes \ket{\boldsymbol{0}})$:

\begin{equation}
    \label{eq:lower_bound}
    S \geq \alpha^k (d^2 - 1)^k (2 \beta)^{N_{FC}},
\end{equation}{}
where $N_{FC}$ is the number of two-qubit blocks in the future cone of the Pauli string $h$.

For $L$ layers and an ansatz with coordination number $z$, $N_{FC} \sim k L^{2z}$, at least until the future cone spreads to the entire ansatz.

\textbf{Potential caveat:} the sum we consider consists of both positive and negative terms. What if the process of repeated application of $M_2$ decreases the positive ones while keeping the negative ones intact? If something like that happens, the lower bound may not hold.

***

There is a separate discussion about approximate $t$-designs and \textit{tensor product expanders}. For these, one needs to look at the superoperator $\Delta_{\nu, t}$ on $\mc{L}(\mc{H}^{\otimes t})$:

\begin{equation}
    \Delta_{\nu, t} [A] = \int U^{\otimes t} A (U^\dagger)^{\otimes t} d\nu (U).
\end{equation}{}

I'll omit the exact definitions for now, but $\nu$ is a $t$-tensor product expander if that superoperator is close to the superoperator $\Delta_{\mu_{Haar}, t}$ defined in the same fashion for the Haar measure. The closeness here is meant in the sense of the (super)operator norm.

The distribution is an $\epsilon$-approximate $t$-design if the follwing is true:

\begin{equation}
    (1 -\epsilon) \Delta_{\mu_{Haar}, t} \preceq \Delta_{\nu, t} \preceq (1 + \epsilon) \Delta_{\mu_{Haar}, t},
\end{equation}{}
where $\mc{A} \preceq \mc{B}$ means that $\mc{B} - \mc{A}$ is a completely positive channel.

I'm not using these two definitions for anything yet, but an interested reader can refer to (Brandao et al, 2016) for more details.

\section{Onset of the barren plateaus for a two-local ansatz}

In this section, we will consider ans\"atze consisting only of 2-local qubit gates. To make meaningful results, we will need to use (\ref{eq:int_haar}) and provide examples of the action of $M_{\mc{Y}}$ for different possible inputs.

\begin{enumerate}
    \item A pair of Pauli strings $\sigma_\alpha \otimes \sigma_\beta$. Proposition \ref{prop:paulis_decouple} allows us to only consider the Pauli matrices that match over the different copies: $A = B = \sigma_\alpha \otimes \sigma_\beta$. Traces of $A$ and $B$ vanish, but $\Tr AB = d^2$, hence we obtain 
    $\frac{1}{d^4 - 1}(-\mathbbm{1}_{d^2} + d^2 \mc{S})$.
    \item Inputs of the form $\mathbbm{1} \otimes \sigma_\alpha$. Just like in the previous case, $\Tr AB = d^2, \Tr A = \Tr B = 0$, and the result is the same.
    \item Identity on each qubit or swap on all qubit pairs. These operators are unaffected due to Proposition \ref{prop:m2_is_proj}.
    \item A mixture of identity and swap gates: $\mathbbm{1}_{1, 1'} \otimes \mc{S}_{2, 2'}$. Here we may decompose the swap gate as a sum of Pauli matrix pairs, but a more clear way is to use (\ref{eq:int_haar_swap}) with $C = \mathbbm{1}_{1, 1'} \otimes \mc{S}_{2, 2'}$. Evidently, $\Tr C = \Tr \mc{S}_{(1, 2), (1', 2')} C  = d^3$, where $(1, 2)$ denotes the Hilbert space spanned by the two qudits. Contracting all the factors yields $M_{(1, 2), (1', 2')}(\mathbbm{1}_{1, 1'} \otimes \mc{S}_{2, 2'}) =
    \frac{d}{d^2+1}(\mathbbm{1}_{(1, 2), (1', 2')} + \mc{S}_{(1, 2), (1', 2')})$.
    \item A mixture of Pauli gates and a swap: $\sigma_{\alpha_1} \otimes \sigma_{\alpha_{1'}} \otimes \mc{S}_{2, 2'}$. Here $\Tr C = 0, \ \Tr \mc{S} C = d^3.$ Overall, we get $\frac{d}{d^4-1}( d^2 \mc{S}_{(1, 2), (1', 2')} - \mathbbm{1}_{(1, 2), (1', 2')})$
\end{enumerate}

Now we can consider how the quantity $\mathrm{V}$ changes when we add more and more layers to the ansatz. First, due to proposition \ref{prop:paulis_decouple} we can assume without loss of generality that $H$ is a single Pauli string. Now, let the support of $H$ overlap with $K_1$ gates from the first layer. Then, each of those $K_1$ gates acts on $H$ via the $M$ operator with the corresponding support. $H$ decomposes into $2^{K_1}$ terms consisting of identities and swaps (and possibly some Pauli matrices not covered by the first layer). The sum of the coefficients will then be equal to 
\begin{equation}
\label{eq:single_layer_plateau}
    \mathrm{V}_1 = \left(\frac{d^2 - 1}{d^4 - 1}\right)^{K_1} = (d^2 + 1)^{-K_1}.
\end{equation}{}

\begin{remark}
This may be the one of the most important takeaways of this paper. If we ignore the matter of the commutator for the time being, this part gives a way to explain the onset of the plateau for one layer. An Ising or Heisenberg Hamiltonian consists entirely of 2-local terms. For such Pauli string, $K_1 \in {1, 2}$. For a Hamiltonian $H = Z \otimes Z \otimes \dots \otimes Z$, $K_1 = \lfloor \frac{n}{2} \rfloor$. The same goes for $H_{proj} = \ket{000...0} \bra{000...0}$, although the factor is different since this is not the same as a Pauli string. Partially, this confirms the observation of [Cerezo et al] that for very nonlocal Hamiltonians, the plateau sets on even after one layer of the ansatz. However, this also hints that geometric locality of the ansatz is also at play. For example, $H = Z \otimes \mathbbm{1} \otimes Z \otimes \mathbbm{1} ...$, attacked with a checkerboard ansatz, should exhibit the same behavior, even though it is $n/2$-local and not $n$-local.
\end{remark}{}


\textbf{Important point:} I am now not sure how to extend this, so let us for now assume that all support of $H$ is covered by the first layer of the ansatz.

% Next, let us also consider all gates from the subsequent layers that are necessary to cover all the remaining qubits where $H$ acts nontrivially. For example, if we had a 5-qubit registry and covered qubits (1, 2), (3, 4) in the first layer, then we would take the first gate that acts on qubit 5. Any new extra gate like this meets only the inputs of of the forms listed above under points 2 and 5. Each term splits into two terms, with the sum of the two being the old coefficient times either $(d^3 - 1)$ or $(d^2 - 1)$. So, if we added $K_2$ such gates in the process, we can estimate the sum of absolute values of coefficients: 

% Further on, let us see what may happen to the sum of the coefficients when subsequent gates are applied. For each term, there are the same possible inputs as explained above, except 1. 

Now comes a point where I do not know how to proceed. At this point, $H$ is already transformed into a sum of terms consisting entirely of identity and swap operators. Any next two-qubit gate can only meet a pair of identity operators, a pair of swap operators, or an identity-swap pair. In the latter case, if the coefficient of a term was $c$, then the resulting two terms will have the sum of coefficients equal to $c \cdot \frac{2d}{d^2 + 1}$. In the two former cases, the term is unchanged. So, for each term after the first layer, we can lower bound the magnitude of its input into the final sum:

\begin{equation}
    |c_{final}| \geq |c| \left( \frac{2d}{d^2 + 1}\right)^{\#FC},
\end{equation}{}
where $\#FC$ is the number of gates that will act nontrivially on that term or any of its descendants (the ``future cone''). 
If all summands yielding $\mathrm{V}$ were positive, we would be done here. However, there are both positive and negative terms in the overall expression. To lower bound $\mathrm{V}$, we need to lower bound the positive terms and upper bound the negative terms. The latter is the missing point that I need to make this work complete.

\subsection{commutator}

When the input of $\mc{C}$ is a Pauli string, the output is straightforward. It is more interesting to consider what happens when a swap operator is sent as input (see Fig. N). Let's see what happens if we assume that all support of $iF$ is swapped:

\begin{equation}
\label{eq:commutator_swap}
    \begin{aligned}
         ([iF, \cdot] \otimes [iF, \cdot]) \mc{S} & = iF_{\mc{Y}} (iF_{\mc{Y'}} \mc{S} - \mc{S} iF_{\mc{Y'}}) - 
        (iF_{\mc{Y'}} \mc{S} - \mc{S} iF_{\mc{Y'}}) iF_{\mc{Y}} = \\
        & = \mc{S} \left( 2 (iF_{\mc{Y}}) (iF_{\mc{Y'}})  - (iF_{\mc{Y}})^2 - (iF_{\mc{Y'}})^2\right).
    \end{aligned}{}
\end{equation}{}

Let's keep this guy for future reference as we will need to plug it to $M$.

\subsection{Ising model}

Consider one Pauli string out of the Ising model, acting on spins 1, 2. We will denote the corresponding paired string as $h \otimes h=zz1111$. Now, act on it with $\mc{M}_{(1, 2)}$:

$$
h \otimes h \mapsto h_1  = \alpha (d^2 ss1111 - 111111).
$$

All other gates in the first layer of the ansatz will change nothing.
Next layer:

$$
h_2  = \mc{M}_{2, 3} (h_1) = \alpha (d^2 \beta (sss111 + s11111) - 111111).
$$

We are only interested in the sum of the coefficients, but the number of terms is quickly getting out of control as we apply more operators.



% \begin{proof}
% 1. First apply the commutator:
% \begin{equation}
%     [iX, \cdot ]^{\otimes 2} (x + y + z) = i^2 (2iZ)^{\otimes 2} + i^2 (-2iY)^{\otimes 2} = 4z + 4y.
% \end{equation}{}
% Next, apply the mixing operator:
% \begin{equation}
%     M(4z + 4y) = 4M(z) + 4 M(y) = 8M(y) = \frac{8}{3} (x+y+z).
% \end{equation}{}

% 2. We know that the output of $M$ is equal to
% $$\frac{1}{15}\left(
% \sum_{i,j} (\sigma_i \otimes \sigma_j)^{\otimes 2}
% + \sum_{i} (\sigma_i \otimes 1)^{\otimes 2}
% + \sum_{j} (1 \otimes \sigma_j)^{\otimes 2}
% \right).$$

% We calculate this:

% \begin{multline}
%     [i \sigma_\alpha \otimes \sigma_\beta, \cdot ]^{\otimes 2} \cdot (\sigma_1 \otimes \sigma_2)^{\otimes 2} = [i \sigma_\alpha \otimes \sigma_\beta, \sigma_1 \otimes \sigma_2]^{\otimes 2} = \\
%     = (4i \cdot i\epsilon_{\alpha 1 \gamma} i\epsilon_{\beta 1 \gamma'})^2 (\sigma_\gamma \otimes \sigma_{\gamma'})^{\otimes 2} = 16(\epsilon_{\alpha 1 \gamma} \epsilon_{\beta 1 \gamma'})^2 (\sigma_\gamma \otimes \sigma_{\gamma'})^{\otimes 2}
% \end{multline}{}
% So, most of the terms vanish, and we get $[i \sigma_\alpha \otimes \sigma_\beta, \cdot ] \circ M\left( (\sigma_1 \otimes \sigma_2)^{\otimes 2}\right) = \frac{16}{15} \sum_{i \neq \alpha, j \neq \beta} (\sigma_i \otimes \sigma_j)^{\otimes 2}$. Finally, applying and extra $M$ yields:
% $$
% M \circ [i \sigma_\alpha \otimes \sigma_\beta, \cdot ] \circ M\left( (\sigma_1 \otimes \sigma_2)^{\otimes 2}\right) = \frac{64}{15} M\left( (\sigma_1 \otimes \sigma_2)^{\otimes 2}\right)
% $$

% \end{proof}{}




% \subsection{Fancy shorthand notation}

% We know that all ``double Hamiltonians'' that come out of our process consist exclusively of identities and swaps. We also know that the $M$ operator treats all Pauli matrices equally (more like, all conjugate classes of $SU(d)$?). So, e can denote all relevant ``double Hamiltonians'' by strings like that: $H \sim 11s\sigma\sigma$, which means that this Hamiltonian acts on five pairs of qubits, swapping qubits 3 and 3', and acting with some Pauli matrices on qubits 4, 4', 5, 5'.

% Let us introduce the following notation: any paired Pauli string $h \otimes h$ acting on $n$ pairs of qubits will be written using $n$ symbols. When we write a lowercase Latin letter of a Pauli matrix in the $i$'th symbol (e.g. $z$), we mean that this Pauli matrix acts on the qubits $i, i'$. Thus, a paired Pauli string 
% $(X \otimes Y \otimes \mathbbm{1} \otimes \mathbbm{1})^{\otimes 2}$ will be written as $xy11$. Let us also denote by $s$ a swap gate acting on qubits $i, i'$. Thus, in the output of the local mixing operators, as in the conditions of Theorem \ref{thm:all_are_ids_and_swaps}, will be written as many strings consisting of symbols $1$ and $s$. For example, 
% $\mc{M}_{1, 2} (xy11) = \alpha (d^2 ss11 - 1111)$.

% \textbf{I plan to remove all fancy notation below.}

% Let us introduce the following notation: any paired Pauli string $h \otimes h$ acting on $n$ pairs of qubits will be written using $n$ symbols. When we write a lowercase Latin letter of a Pauli matrix in the $i$'th symbol (e.g. $z$), we mean that this Pauli matrix acts on the qubits $i, i'$. Thus, a paired Pauli string 
% $(X \otimes Y \otimes \mathbbm{1} \otimes \mathbbm{1})^{\otimes 2}$ will be written as $xy11$. Let us also denote by $s$ a swap gate acting on qubits $i, i'$. Of course, an operator with such a swap is not a paired Pauli string.
% % Thus, in the output of the local mixing operators, as in the conditions of Theorem \ref{thm:all_are_ids_and_swaps}, will be written as many strings consisting of symbols $1$ and $s$. For example, 
% % $\mc{M}_{1, 2} (xy11) = \alpha (d^2 ss11 - 1111)$.

% Finally, for $d=2$ define $\varphi = \frac{1}{3}(2s - 1) = \frac{1}{3} (x+y+z)$.
